The Gravity of Classical Fields: And Its Effect on the Dynamics of Gravitational Systems

Classical fields are ubiquitous in theoretical physics. They find applications in almost all areas of physics, from condensed matter and particle physics to cosmology and astrophysics. Scalar fields, in particular, can give rise to confined structures, such as boson stars, oscillatons or Q-balls. These objects are interesting hypothetical new "dark matter stars", but also good descriptions of dark matter cores when the fields are ultralight. In this thesis, we study the dynamical response of such confined bosonic structures when excited by external matter (stars, planets or black holes) in their vicinities. Such perturbers can either be piercing through the bosonic configuration or undergoing periodic motion at its center (e.g., binaries). Our setup can also efficiently describe the interaction between a moving massive black hole and the surrounding environment. It also depicts dark matter depletion as a reaction to an inspiralling binary within a dark matter core. Our results provide a complete picture of the interaction between black holes or stars and the ultralight dark matter core environment where they may live in. This thesis also deals with several classical field environmental effects on the motion (or, ultimately, the survival) of compact objects, like black holes.

==> Chapters/Chapter01.tex <==
%************************************************
\chapter{Introduction}\label{ch:introduction}
%************************************************

aa


%*****************************************
%*****************************************
%*****************************************
%*****************************************
%*****************************************


==> Chapters/Chapter03.tex <==
%************************************************
\chapter{Stirring up ultralight dark matter}\label{ch:mathtest} 
%************************************************


%*****************************************
%*****************************************
%*****************************************
%*****************************************
%*****************************************


==> Chapters/ch_SR.tex <==
%************************************************
\chapter{Newtonian Boson Stars}\label{ch:nbs}
%************************************************

aa


%*****************************************
%*****************************************
%*****************************************
%*****************************************
%*****************************************


==> FrontBackmatter/Declaration.tex <==
%*******************************************************
% Declaration
%*******************************************************
\pdfbookmark[0]{Declaration}{declaration}
\chapter*{Declaration}
\thispagestyle{empty}

I declare that this document is an original work of my own and that it fulfills all the requirements of the Code of Conduct and Good Practices of the Universidade de Lisboa.
\bigskip
\vspace{5mm}

\noindent Name:\\
\noindent Student number: \\
\bigskip
\vspace{5mm}

\noindent\textit{\myLocation, \myTime}

\smallskip

\begin{flushright}
    \begin{tabular}{m{6cm}}
        \\ \hline
        \centering\myName \\
    \end{tabular}
\end{flushright}

